An adaptive IGA-BEM with hierarchical B-splines based on quasi-interpolation quadrature schemes

The isogeometric formulation of Boundary Element Method (BEM) is investigated within the adaptivity framework. Suitable weighted quadrature rules to evaluate integrals appearing in the Galerkin BEM formulation of 2D Laplace model problems are introduced. The new quadrature schemes are based on a spline quasi-interpolant (QI) operator and properly framed in the hierarchical setting. The local nature of the QI perfectly fits with hierarchical spline constructions and leads to an efficient and accurate numerical scheme. An automatic adaptive refinement strategy is driven by a residual based error estimator. Numerical examples show that the optimal convergence rate of the BEM solution is recovered by the proposed adaptive method.

==> Intro.tex <==
% section 1: INTRODUCTION
Boundary Element Methods (BEMs) are methods studied since the mid 1980s for the numerical solution of those Boundary Value Problems (BVPs), which can be transformed into Boundary Integral Equations (BIEs), see, e.g., \cite{BEMbook} for a recent overview. A common reference example is the Laplacian differential operator, but the theory can be extended also to more general partial differential equations, like the Helmholtz equation and the Stokes equations, which have applications in acoustics and fluid dynamics, respectively.

Boundary element methods have two main advantages: the dimension reduction of the computational domain and the simplicity for treating external problems. As a major drawback, the resulting integrals can be singular and therefore
robust and accurate quadrature formulas are necessary for their numerical computation. The solution is then obtained by collocation or Galerkin procedures.
 
 
The advent of \emph{Isogeometric Analysis} (IgA) \cite{ref2,LibroHughes} has brought a renewed interest in BEMs. In the IgA approach, a tight relation between the geometry of the domain and the representation of the approximate solution of the differential problem is established. In particular, IgA relies on a spline description of the domain, which is standard in Computer Aided Design (CAD), and on the usage of (possibly generalized and refined) analogous   spaces for the discretization of the differential problem.

In order to reduce complexity and gain efficiency, the use of collocation \cite{TauRodHug} or mixed collocation is the most common solution, see, e.g., \cite{Ginnis,  Simp2012}.
Indeed the Galerkin method has been generally avoided because it requires a double integration process, which appear difficult to evaluate efficiently. There are however applications, for example in crack propagation
problems, elasticity, elastodynamics, etc., where the use of a
Galerkin method may give some important advantages. Papers  using the IgA Galerkin BEM approach can be found in the literature, dealing with problems in acoustics \cite{Coox, SimpsonScott} or  flows \cite{politis, Joneidi}. BEM formulation has been used also to construct computational domains for Galerkin-IgA \cite{Falini}.
Recently, the IgA paradigm has been combined for the first time to the Symmetric Galerkin Boundary Element Method (IgA-SGBEM)\cite{ADSS1, ADSS2, Nguyen16}, which has revealed to be very effective among BEM schemes. Moreover, the full potential of B-splines over the more common Lagrangian basis has been recently exploited in \cite{ACDS3}.

%Clearly, also in the BEM context
When dealing with problems characterized by solutions with sharp features, adaptivity is a key ingredient to efficiently solve them; it requires suitable error estimations, as well as efficient local refinement procedures. While adaptive BEM have been widely studied in the literature, see, e.g., \cite{feischl2015arcme} for a recent review, the theory of adaptivity for isogeometric boundary element methods is still at a preliminary stage. A posteriori error analysis and refinement algorithms in the 2D setting have been presented in \cite{feischl2015reliable,feischl2016}. In \cite{feischl2017}, the optimal convergence of adaptive IgA-BEM for weakly singular equations was also proven. In all these studies, the adaptive scheme relies on the locally refinable nature of classical univariate B-splines, the standard spline basis adopted in CAD and IgA. In higher dimensions, however, the tensor-product B-spline structure does not provide local refinement capabilities and alternative spline spaces need to be considered.

One of the prominent approaches in the design and analysis of adaptive isogeometric methods exploits the multilevel structure of hierarchical B-splines, see, e.g., \cite{vuong2011}. A hierarchical B-spline space is constructed from a nested sequence of B-spline spaces, defined on different levels of resolution and on %considers B-splines defined on a domain hierarchy that identifies an increasing level of resolution in
strictly localized parts of the domain. Non-uniform mesh configurations can be considered at different hierarchical levels. However, the adaptive nature of the spline hierarchy is usually considered on nested sequences of dyadically refined knots to simplify and speed up computations, while simultaneously providing an efficient adaptive framework. For the same reasons, the uniform configuration of hierarchical spline spaces based on a dyadic refinement is attractive also for a numerical treatment of 2D problems in the adaptive BEM.
\medskip

In this paper we present an adaptive IgA-BEM with hierarchical B-splines based on local quadrature schemes to solve 2D Laplace problems. The uniform structure of B-splines at different levels can be properly exploited in the assembly of the discretization matrices. In particular, the new quadrature schemes based on spline quasi--interpolation %\cite{CFSS18}
are investigated in this paper in the context of boundary integral equations and properly framed in the hierarchical setting.

The term {\it quasi--interpolation} (\emph{QI}) denotes a general approach to construct efficient local approximants to a given set of data or a given function; see \cite{LS75} for a general introduction to spline quasi--interpolation.
The quadrature rules adopted here are based on a quasi--interpolation operator firstly introduced in \cite{MSbit09} and applied to non singular numerical integration in \cite{MS12}. Then, the same QI-based idea was adopted in \cite{CFSS18} to develop efficient and competitive quadratures for singular integrals appearing in the IgA-BEM context.   The rule is effective also for nearly singular integrals.
Although the use of spline quasi--interpolation for numerical integration was already studied in several papers \cite{rabinowitz1990numerical, dagnino1993numerical, dagnino1997product, demichelis1996quasi}, its introduction in the IgA context is a novelty. In particular, in this work, the QI formulas derived in \cite{MS12} and \cite{CFSS18} are integrated in a Galerkin BEM model and suitably framed into a hierarchical adaptive scheme. In fact, the Galerkin Boundary Element Method is combined with an automatic adaptive refinement strategy driven by a residual based error estimator.  Numerical examples show the optimal convergence rates achieved by the hierarchical isogeometric scheme.
%}

%Different QI schemes:
%In \cite{AllSab10} the authors introduce a QI scheme based on quasi--Lagrange splines and for a uniform partition with elements length $h$, prove the optimal order $O(h^{m+1})$ for a smooth kernel and an integrand function $g\in C^{m+1}$; order $O(h^{m+1}\log h)$ for a logarithmic kernel and again $g\in C^{m+1}$. In \cite{Sabit10} a quadrature formula based on a quartic spline quasi--interpolant operator introduced by the first author in \cite{sablonniere2005univariate} is investigated. In \cite{sablonniere2012high} a class of quadrature rules with end-point corrections based on integrating spline quasi--interpolants are introduced.  The correction weights are obtained as solutions of
%certain systems of linear algebraic equations.}

The structure of the paper is as follows. Section~\ref{sec:sgbem} presents the integral formulation of the model problem. Section~\ref{sec:bsplines} introduces B-spline representations of the domain boundary, commonly used in computer aided design systems. Hierarchical spline constructions and the definition of the isogeometric discretization are reviewed in Section~\ref{sub:hier} and \ref{sec:iga}, respectively. The adaptive scheme is summarized in Section~\ref{sec:adapt}. Section~\ref{sec:quad} introduces the quadrature formulas based on spline quasi--interpolation. In Section~\ref{sec:num} the developed  model is applied to an exterior and two interior 2D Laplace problems, all  suited for adaptivity. Finally, Section~\ref{sec:conc} concludes the paper.


